Unbiased variance reduction in randomized experiments

This paper develops a flexible method for decreasing the variance of estimators for complex experiment effect metrics (e.g. ratio metrics) while retaining asymptotic unbiasedness. This method uses the auxiliary information about the experiment units to decrease the variance. The method can incorporate almost any arbitrary predictive model (e.g. linear regression, regularization, neural networks) to adjust the estimators. The adjustment involves some free parameters which can be optimized to achieve the smallest variance reduction given the predictive model performance. Also we approximate the achievable reduction in variance in fairly general settings mathematically. Finally, we use simulations to show the method works.

==> pred_accuracy_infodf_alldatanoexptid_v18.tex <==
% latex table generated in R 3.4.1 by xtable 1.8-2 package
% Mon Jan 14 11:16:40 2019
\begin{table}[ht]
\centering
\begin{tabular}{|r|l|r|r|r|}
  \hline
 & model\_formula & cv\_cor & theta & sd\_ratio \\
  \hline
1 & imp\_count: gender+country & -0.02 & 0.00 & 1.00 \\
  2 & obs\_interact: gender+country & -0.01 & 0.00 & 1.00 \\
  3 & obs\_amount: gender+country & -0.02 & 0.00 & 1.00 \\
   \hline
\end{tabular}
\caption{Prediction accuracy for various responses when using all the data in building the model and no experiment label.} 
\label{pred_accuracy_infoDf_allDataNoExptId_v18}
\end{table}


==> pred_accuracy_infodf_alldatanoexptid_v19.tex <==
% latex table generated in R 3.4.1 by xtable 1.8-2 package
% Mon Jan 14 13:09:27 2019
\begin{table}[ht]
\centering
\begin{tabular}{|r|l|r|r|r|}
  \hline
 & model\_formula & cv\_cor & theta & sd\_ratio \\ 
  \hline
1 & imp\_count: gender+country & 0.39 & 0.96 & 0.92 \\ 
  2 & obs\_interact: gender+country & 0.48 & 1.00 & 0.88 \\ 
  3 & obs\_amount: gender+country & 0.46 & 1.00 & 0.89 \\ 
   \hline
\end{tabular}
\caption{pred accuracy infoDf allDataNoExptId v19} 
\label{pred_accuracy_infoDf_allDataNoExptId_v19}
\end{table}


==> pred_accuracy_infodf_contdataonly_v19.tex <==
% latex table generated in R 3.4.1 by xtable 1.8-2 package
% Mon Jan 14 13:09:26 2019
\begin{table}[ht]
\centering
\begin{tabular}{|r|l|r|r|r|}
  \hline
 & model\_formula & cv\_cor & theta & sd\_ratio \\ 
  \hline
1 & imp\_count: gender+country & 0.42 & 1.00 & 0.91 \\ 
  2 & obs\_interact: gender+country & 0.50 & 1.00 & 0.86 \\ 
  3 & obs\_amount: gender+country & 0.45 & 0.96 & 0.89 \\ 
   \hline
\end{tabular}
\caption{pred accuracy infoDf contDataOnly v19} 
\label{pred_accuracy_infoDf_contDataOnly_v19}
\end{table}


==> pred_accuracy_infodf_withexptdata_v18.tex <==
% latex table generated in R 3.4.1 by xtable 1.8-2 package
% Tue Jul  3 11:46:30 2018
\begin{table}[ht]
\centering
\begin{tabular}{|r|l|r|r|r|}
  \hline
 & model\_formula & cv\_cor & theta & sd\_ratio \\ 
  \hline
1 & imp\_count: gender+country+expt\_id & 0.14 & 0.91 & 0.99 \\ 
  2 & obs\_interact: gender+country+expt\_id & 0.21 & 1.00 & 0.98 \\ 
  3 & obs\_amount: gender+country+expt\_id & 0.22 & 1.00 & 0.98 \\ 
   \hline
\end{tabular}
\caption{Prediction power using model fitted with all data (including treatment) only.} 
\label{pred_accuracy_infoDf_withExptData_v18}
\end{table}


==> pred_accuracy_infodf_withexptdata_v19.tex <==
% latex table generated in R 3.4.1 by xtable 1.8-2 package
% Fri Jul  6 12:32:50 2018
\begin{table}[ht]
\centering
\begin{tabular}{|r|l|r|r|r|}
  \hline
 & model\_formula & cv\_cor & theta & sd\_ratio \\ 
  \hline
1 & imp\_count: gender+country+expt\_id & 0.46 & 1.00 & 0.89 \\ 
  2 & obs\_interact: gender+country+expt\_id & 0.52 & 0.97 & 0.85 \\ 
  3 & obs\_amount: gender+country+expt\_id & 0.51 & 1.00 & 0.86 \\ 
   \hline
\end{tabular}
\caption{Prediction power using model fitted with all data (including treatment) only.} 
\label{pred_accuracy_infoDf_withExptData_v19}
\end{table}


==> pred_accuracy_infodf_withtreatdata_v19.tex <==
% latex table generated in R 3.4.1 by xtable 1.8-2 package
% Mon Jan 14 13:09:27 2019
\begin{table}[ht]
\centering
\begin{tabular}{|r|l|r|r|r|}
  \hline
 & model\_formula & cv\_cor & theta & sd\_ratio \\ 
  \hline
1 & imp\_count: gender+country+expt\_id & 0.43 & 0.94 & 0.90 \\ 
  2 & obs\_interact: gender+country+expt\_id & 0.53 & 0.98 & 0.85 \\ 
  3 & obs\_amount: gender+country+expt\_id & 0.51 & 1.00 & 0.86 \\ 
   \hline
\end{tabular}
\caption{pred accuracy infoDf withTreatData v19} 
\label{pred_accuracy_infoDf_withTreatData_v19}
\end{table}

